Multi-Parameter Mechanisms for Consumer Surplus Maximization

We consider the problem of designing auctions which maximize consumer surplus (i.e., the social welfare minus the payments charged to the buyers). In the consumer surplus maximization problem, a seller with a set of goods faces a set of strategic buyers with private values, each of whom aims to maximize their own individual utility. The seller, in contrast, aims to allocate the goods in a way which maximizes the total buyer utility. The seller must then elicit the values of the buyers in order to decide what goods to award each buyer. The canonical approach in mechanism design to ensure truthful reporting of the private information is to find appropriate prices to charge each buyer in order to align their objective with the objective of the seller. Indeed, there are many celebrated results to this end when the seller's objective is welfare maximization [Clarke, 1971, Groves, 1973, Vickrey, 1961] or revenue maximization [Myerson, 1981]. However, in the case of consumer surplus maximization the picture is less clear -- using high payments to ensure the highest value bidders are served necessarily decreases their surplus utility, but using low payments may lead the seller into serving lower value bidders. Our main result in this paper is a framework for designing mechanisms which maximize consumer surplus. We instantiate our framework in a variety of canonical multi-parameter auction settings (i.e., unit-demand bidders with heterogeneous items, multi-unit auctions, and auctions with divisible goods) and use it to design auctions achieving consumer surplus with optimal approximation guarantees against the total social welfare. Along the way, we answer an open question posed by Hartline and Roughgarden [2008] for the two bidders single item setting.

==> omitted-proofs-unit-demand.tex <==
\begin{proof}[Proof of Lemma~\ref{shared-bound}]
    Consider the allocation rule $\AllocRule$: For a valuation profile $v$, $\AllocRule$ allocates each item $j$ to one of the agents in $\MostValuableAgents{j}$ uniformly at random.    
    To prove this lemma we bound the expected social welfare by the expected welfare of the allocation rule $\AllocRule$.
    The expected welfare of an agent $i$ under allocation rule $\AllocRule$ is equal to $\E_{v \sim \mathcal{F}}\left[\frac{v_i(\{\MostValuableItem{i}\})}{|\MostValuableAgents{\MostValuableItem{i}}|}\right]$. We next analyze the random variable of $|\MostValuableAgents{\MostValuableItem{i}}|$. We know that by definition $i \in\MostValuableAgents{\MostValuableItem{i}}$, and 
    by the \assumption assumption we have that for every $
    i'\in \agents \setminus \{i\}$, it holds that $\Pr[i'\in \MostValuableAgents{\MostValuableItem{i}} ] = \frac{1}{m}$. Combining with the independent assumption, we get that  $\mid \MostValuableAgents{\MostValuableItem{i}}\mid $ is distributed as  
      $1+ Bin(n-1, \frac{1}{m})$. Next we analyze the expected value of  $\frac{1}{\mid \MostValuableAgents{\MostValuableItem{i}}\mid}$.

    \begin{align} \label{expected_value_pr_getting_item}
        \begin{aligned}
        \E\left[\frac{1}{\mid \MostValuableAgents{\MostValuableItem{i}}\mid}\right]& =\sum_{k=0}^{n-1}\frac{1}{k+1}\binom{n-1}{k}(\frac{1}{m})^k\cdot(1-\frac{1}{m})^{n-1-k}  \\
        &= \sum_{k=0}^{n-1}\frac{1}{n}\binom{n}{k+1}(\frac{1}{m})^{k}\cdot(1-\frac{1}{m})^{n-(k+1)} \\ &= \frac{m}{n}\sum_{k=0}^{n-1}\binom{n}{k+1}(\frac{1}{m})^{k+1}\cdot(1-\frac{1}{m})^{n-(k+1)}\\ 
        & = \frac{m}{n}\cdot(1-(1-\frac{1}{m})^{n}),
        \end{aligned}
    \end{align}
    where the second equality is due to the identity $\binom{n}{k} = \frac{n}{k}\binom{n-1}{k-1}$. The Last equality follows by observing that $\sum_{k=0}^{n-1}\binom{n}{k+1}(\frac{1}{m})^{k+1}\cdot(1-\frac{1}{m})^{n-(k+1)}$ is equal to the probability that a binomial random variable with parameters $n$ and $\frac{1}{m}$ equals to some $k$ between $1$ and $n$, i.e., it equals to the probability that a binomial random variable with parameters $n$ and $\frac{1}{m}$ is not equal to $0$.

By the independence assumption we get that $v_i(\{\MostValuableItem{i}\})$ is independent of $|\MostValuableAgents{\MostValuableItem{i}}|$ which implies that:
\begin{equation}
    \E_{v \sim \mathcal{F}}\left[\frac{v_i(\{\MostValuableItem{i}\})}{|\MostValuableAgents{\MostValuableItem{i}}|}\right] = \E_{v \sim \mathcal{F}}[v_i(\{\MostValuableItem{i}\})]\cdot \E_{v \sim \mathcal{F}}\left[\frac{1}{|\MostValuableAgents{\MostValuableItem{i}}|}\right]. \label{eq:v-ind} 
\end{equation}
    Thus, by combining Equation~\ref{expected_value_pr_getting_item} and Equation~\ref{eq:v-ind} we get that the expected welfare of the allocation rule $\AllocRule$ is: 
    $$\E_{v\sim\mathcal{F}}[\sum_{i \in \agents } v_i(\{\MostValuableItem{i}\})]\cdot  \frac{m}{n}\cdot(1-(1-\frac{1}{m})^{n}).$$
    Now, we split the analysis depending on whether $n \geq m$, or $ n<m$.

    \paragraph{Case 1: $n\geq m$.} In this case $ \frac{m}{n}\cdot(1-(1-\frac{1}{m})^{n}) \geq \frac{m}{n}\cdot(1-(1-\frac{1}{m})^{m}) \geq \frac{m}{n}\cdot(1-\frac{1}{e})$, and so we get:
    $$
    \E_{v\sim\mathcal{F}}[\sw{\agents}{\items}] %\geq \E_{v\sim\mathcal{F}}[\sum_{i \in \agents } v_i(\{\MostValuableItem{i}\})]\cdot  \frac{m}{n}\cdot(1-(1-\frac{1}{m})^{n})
    \geq  \E_{v\sim\mathcal{F}}[\sum_{i \in \agents } v_i(\{\MostValuableItem{i}\})]\cdot  \frac{m}{n} \cdot (1-\frac{1}{e}).
    $$
    \paragraph{Case 2: $n < m$.} In this case $ \frac{m}{n}\cdot(1-(1-\frac{1}{m})^{n}) \geq \frac{m}{n}\cdot(1-\frac{1}{e}^{\frac{n}{m}})$. Let $f(x)= x\cdot(1-e^{-\frac{1}{x}})$, and observe that this is an increasing function for $x \geq 0$. Since $n<m$, we have that $ \frac{m}{n}\cdot(1-\frac{1}{e}^{\frac{n}{m}}) >f(1) = 1-\frac{1}{e}$. Overall:
    $$
    \E_{v\sim\mathcal{F}}[\sw{\agents}{\items}] \geq \E_{v\sim\mathcal{F}}[\sum_{i \in \agents } v_i(\{\MostValuableItem{i}\})]\cdot  \frac{m}{n}\cdot(1-(1-\frac{1}{m})^{n}) \geq  \E_{v\sim\mathcal{F}}[\sum_{i \in \agents } v_i(\{\MostValuableItem{i}\})]\cdot (1-\frac{1}{e}).
    $$
    This concludes the proof of the lemma.    
\end{proof}

==> unit-demand.tex <==
\newcommand{\MostValuableAgentsMap}{\mu^{-1}_{v}}
\newcommand{\MostValuableAgents}[1]{\mu^{-1}_{v}(#1)}
\newcommand{\MostValuableItemMap}{\mu_{v}}
\newcommand{\MostValuableItem}[1]{\mu_{v}(#1)}
\newcommand{\copiesmoreagents}{\log\frac{n\cdot (\frac{2e}{e-1})}{m}}
\newcommand{\copiesmoreagentsTwo}{\frac{n\cdot (\frac{2e}{e-1})}{m}}
\newcommand{\copiesmoreitems}{(\frac{2e}{e-1})}
\newcommand{\sharedconst}{\frac{e}{e-1}}
% \newcommand{\assumption}{uniform highest value }

% \newcommand{\copiesmoreagentsconst}{c}
% \newcommand{\prmoreagents}{0.25}
% \newcommand{\maxagentssamebin}{\frac{7n}{m}}
% \newcommand{\minagentssamebin}{\frac{n}{10m}}
% \newcommand{\minnumofgoodbins}{\frac{m}{10}}
% \newcommand{\prmoreagentsmoreitems}{0.25}
% \newcommand{\minnumofgoodagens}{\frac{n}{10}}
% \newcommand{\maxagentssameitem}{c_1}

% \newcommand{\MaxAngentsSameItemS}{5}
% \newcommand{\MaxAngentsSameItemMinusOS}{4}
% \newcommand{\MinFracNumGoodAngentsS}{\frac{1}{5}}
% \newcommand{\MinNumGoodAngentsS}{n\cdot \frac{1}{5}}
% \newcommand{\PrGS}{0.73}
% \newcommand{\PrNotGS}{0.27}
% \newcommand{\PrAgentBad}{0.21}
% \newcommand{\GoodEventS}{G_2}
% \newcommand{\SetGoodAgents}{G_\agents}
% \newcommand{\AllocRuleS}{a_2}

% \newcommand{\PrItemBad}{0.7}

% \newcommand{\MinAgentsSameItemF}{\frac{n}{10m}}
% \newcommand{\MinAgentsSameItemCoeffF}{\frac{9}{10}}
% \newcommand{\MaxAngentsSameItemF}{\frac{6n}{m}}
% \newcommand{\MaxAngentsSameItemCoeffF}{5}
% \newcommand{\MinGoodItemsF}{\frac{m}{5}}

% \newcommand{\SetGoodItems}{G_\items}
% \newcommand{\GoodEventF}{G_1}
% \newcommand{\AllocRuleF}{a_1}
% \newcommand{\PrGF}{\frac{1}{8}}
% \newcommand{\PrnotGF}{\frac{7}{8}}
% \newcommand{\MinFracGoodAgentsF}{0.02}



\newcommand{\AllocRule}{a}

\subsection{Bayesian Instances }\label{sec:unit-demand}


In this section, we show an improved analysis of the performance of  Mechanism~\ref{algo:vcg-copies} under Bayesian settings. 
In particular, we consider a setting where for each agent $i\in \agents$, his valuation function $v_i:2^{\items} \rightarrow \reals_{\geq 0}$ is drawn from an underlying distribution $F_i$ satisfying the following assumption which we call the \assumption assumption:
For each agent $i$, the probability that an item $j$ is agent $i$'s most valuable item is the same\footnote{If there are multiple items that have the highest value, then the probability is counted only for one of the items. Our mechanism does not use this assumption and can be implemented regardless; we only use this assumption for the surplus guarantee for which it is sufficient that there exists a tie breaking among the items that satisfies the \assumption assumption.} for all items, i.e., for all $j\in\items$ it holds that $\Pr[v_i(
\{j\}) = \max_{j'\in\items} v_i(\{j'\})] = \frac{1}{m}$.
We also assume that the agents' valuations are independent, and we denote by $\mathcal{F} = \mathcal{F}_1 \times \dots \times \mathcal{F}_n$ the product of the agents' distributions. In Bayesian settings, we are interested in maximizing the expected performance of a mechanism, and so we say that a mechanism $M$ guarantees an $\alpha$-approximation (for $\alpha \geq 1$) of the optimal welfare as residual surplus if: $$\E_{v \sim \mathcal{F}}\left[\E_{(A,p)\sim \mech(v_1,\ldots,v_n)} \left[\sum_{i\in\agents} v_i(A_i) - p_i\right]\right] \geq \frac{\E_{v \sim \mathcal{F}}[\sw{\agents}{\items}]}{\alpha}.$$


Our result in this section is that it is possible to extract 
a better fraction of the social welfare as  residual surplus (Theorem~\ref{thm:udB}), generalizing the results of \cite{hartline2008optimal} from the case of identical items to heterogeneous items.
Our result also captures the special case of unit-demand agents where each agent's values are distributed identically and independently from the same distribution, which was studied in \cite{goldner2024simple} concurrently and independently from our work.


% This assumption captures many cases like unit demand agents with i.i.d valuations. We show that for this case   

% when for each agent $i\in\agents$, conditioning on the value of $\max_{j \in \items}v_i(\{j\})$, the probability that each item $j$ is the maximum value item is the same (i.e., $\Pr[v_i(\{j\} = m \mid \max_{j' \in \items}v_i(\{j'\})= m ] = \frac{1}{m}$).  

% We show that for the case of unit-demand valuations,
% when for each agent $i\in\agents$, conditioning on the value of $\max_{j \in \items}v_i(\{j\})$, the probability that each item $j$ is the maximum value item is the same (i.e., $\Pr[v_i(\{j\} = m \mid \max_{j' \in \items}v_i(\{j'\})= m ] = \frac{1}{m}$).  


% the items are identically distributed for each agent\footnote{We assume that each agent $i$ has a distribution $\mathcal{F}_i$, such that the value of agent $i$ for item $j$, for every $j \in \items$, is sampled from $\mathcal{F}_i$ independently at random},

% then it is possible to obtain a better fraction of the social welfare as a residual surplus, generalizing the results of \cite{hartline2008optimal} from the case of identical items to heterogeneous items.

% We note that to obtain the stronger guarantee on the surplus approximation (Theorem~\ref{thm:udB}), we use a weaker assumption on the distribution $\mathcal{F}$, we only require that each agent's most valuable item will be distributed uniformly at random and independently from the other agents.  

% \anote{$\sw{\agents}{\items}$ hides the valuations, and so $\E_{v \sim \mathcal{F}}[\sw{\agents}{\items}]$ might be unclear}



% \subsection{Preliminaries}
\begin{theorem}\label{thm:udB}
    For a set $\items$ of $m$ heterogeneous items, $n$ unit-demand agents $\agents$ with valuations sampled from the distribution $\mathcal{F}$ that satisfies the \assumption assumption, there exists a mechanism whose expected residual surplus is $O(\max\{1, \log \frac{n}{m}\})$ approximation to the welfare as residual surplus.
\end{theorem}


To prove this theorem, we first introduce some notation. 
Let $\MostValuableItemMap:\agents \to \items$ be a mapping from an agent to his most valuable item with respect to a valuation profile $v$, i.e.,   $\MostValuableItem{i} = \arg\max_{j\in \items} v_i(\{j\})$. If an agent $i$ has more than one item with maximal value, we define $\MostValuableItem{i}$ to be one of these items in a way that satisfies that $\Pr_{v_i \sim \mathcal{F}_i}[\MostValuableItem{i}= j]=\frac{1}{m}$, for every item $j \in \items$. Moreover, we assume that agent $i$ breaks ties consistently in an independent way from $v_{-i}$.
Similarly, let $\MostValuableAgentsMap:\items \to 2^\agents$ be a mapping from an item to the set of agents whose most valuable item is this item with respect to a valuation profile $v$, i.e., $\MostValuableAgents{j} = \{ i \mid \MostValuableItem{i}=j\}$. 



% Sometimes we will use the size of the set $\mu^{-1}(j)$ which we denote by $\xi(j) = \mid \mu^{-1}(j) \mid $.  

% for every agent $i\in\agents$, his most valuable item  $\mu(i) = \arg\max_{j\in \items} v_i(\{j\})$, and for every item $j$, $\mu^{-1}(j) = \{ i \mid \mu(i)=j\}$, and $\xi(j) = \mid \mu^{-1}(j) \mid $.

The proof for Theorem \ref{thm:udB} heavily relies on the following lemma:

\begin{lemma}\label{shared-bound}
    It holds that $\E_{v\sim\mathcal{F}}[\sw{\agents}{\items}] \geq \frac{\E{v\sim\mathcal{F}}[\sum_{i \in \agents } v_i(\{\MostValuableItem{i}\})]}{\sharedconst\cdot \max\{{1,\frac{n}{m}\}}}$.
\end{lemma}

% We defer the proof of Lemma~\ref{shared-bound} to Appendix~\ref{app:unB}. Next, we show how to derive Theorem~\ref{thm:udB} from Lemma~\ref{shared-bound}.  

We first show how to derive Theorem~\ref{thm:udB} from Lemma~\ref{shared-bound}, and then we prove Lemma~\ref{shared-bound}.
\begin{proof}[Proof of Theorem~\ref{thm:udB}]
    We prove this theorem by considering Mechanism~\ref{algo:vcg-copies} with parameters $r= \lceil \log_2(\frac{2e}{e-1}\cdot \max\{1, \frac{n}{m}\})\rceil, \, q=1$, and subroutine $B$ for unit demand agents (as defined in \nameref{unit-demand-subroutine}). Now, the expected residual surplus of this mechanism is:

\begin{eqnarray*}
& & \E_{v \sim \mathcal{F}}[\E_{(A,p) \sim \mech(v)}[\sum_{i \in \agents} v_i(A_i) - p_i]] \\ & \geq  & \frac{1}{r+1}\left(\E_{v\sim\mathcal{F}}[\sw{\agents}{ \items}]- \frac{\E_{v\sim\mathcal{F}}[\sw{\agents}{ 2^r\cdot \items}]}{2^r}\right)\\
& \geq & \frac{1}{r+1}\left(\E_{v\sim\mathcal{F}}[\sw{\agents}{ \items}]- \frac{\E_{v\sim\mathcal{F}}[\sum_{i \in \agents } v_i(\{\MostValuableItem{i}\})]}{2^r}\right) \\
& \geq & \frac{1}{r+1}\left(\E_{v\sim\mathcal{F}}[\sw{\agents}{ \items}]- \frac{(\sharedconst\cdot \max\{1, \frac{n}{m}\})\cdot \E_{v\sim\mathcal{F}}[\sw{\agents}{ \items}]}{2^r}\right) \\
% & \geq & \frac{1}{r+1}\left(\E_{v\sim\mathcal{F}}[\sw{\agents}{ \items}](1- \frac{(\sharedconst\cdot \max\{1, \frac{n}{m}\})\cdot \E_{v\sim\mathcal{F}}[\sw{\agents}{ \items}]}{2^r}\right) \\
%& \geq & \frac{1}{r+1}\left(\E_{v\sim\mathcal{F}}[\sw{\agents}{ \items}]- \frac{(\sharedconst\cdot \max\{1, \frac{n}{m}\})\cdot \E_{v\sim\mathcal{F}}[\sw{\agents}{ \items}]}{2^{\log_2(\frac{2e}{e-1}\cdot\max\{1, \frac{n}{m}\})}}\right) \\
& \geq  & \frac{1}{r+1}\cdot\frac{\E_{v\sim\mathcal{F}}[\sw{\agents}{ \items}]}{2},
 \end{eqnarray*}
where the first inequality is due to Lemma~\ref{lem:welfare-guarantee}, the second inequality is since the social welfare of unit-demand agents is always bounded by giving each agent his favorite item, the third inequality is due to Lemma~\ref{shared-bound}, and the last inequality is by assigning the value of $r$.  \end{proof}

Next, we prove Lemma~\ref{shared-bound}.
\begin{proof}[Proof of Lemma~\ref{shared-bound}]
    Consider the allocation rule $\AllocRule$: For a valuation profile $v$, $\AllocRule$ allocates each item $j$ to one of the agents in $\MostValuableAgents{j}$ uniformly at random.    
    To prove this lemma we bound the expected social welfare by the expected welfare of the allocation rule $\AllocRule$.
    The expected welfare of an agent $i$ under allocation rule $\AllocRule$ is equal to $\E_{v \sim \mathcal{F}}\left[\frac{v_i(\{\MostValuableItem{i}\})}{|\MostValuableAgents{\MostValuableItem{i}}|}\right]$. We next analyze the random variable of $|\MostValuableAgents{\MostValuableItem{i}}|$. We know that by definition $i \in\MostValuableAgents{\MostValuableItem{i}}$, and 
    by the \assumption assumption we have that for every $
    i'\in \agents \setminus \{i\}$, it holds that $\Pr[i'\in \MostValuableAgents{\MostValuableItem{i}} ] = \frac{1}{m}$. Combining with the independent assumption, we get that  $\mid \MostValuableAgents{\MostValuableItem{i}}\mid $ is distributed as  
      $1+ Bin(n-1, \frac{1}{m})$. Next we analyze the expected value of  $\frac{1}{\mid \MostValuableAgents{\MostValuableItem{i}}\mid}$.

    \begin{align} \label{expected_value_pr_getting_item}
        \begin{aligned}
        \E\left[\frac{1}{\mid \MostValuableAgents{\MostValuableItem{i}}\mid}\right]& =\sum_{k=0}^{n-1}\frac{1}{k+1}\binom{n-1}{k}(\frac{1}{m})^k\cdot(1-\frac{1}{m})^{n-1-k}  \\
        &= \sum_{k=0}^{n-1}\frac{1}{n}\binom{n}{k+1}(\frac{1}{m})^{k}\cdot(1-\frac{1}{m})^{n-(k+1)} \\ &= \frac{m}{n}\sum_{k=0}^{n-1}\binom{n}{k+1}(\frac{1}{m})^{k+1}\cdot(1-\frac{1}{m})^{n-(k+1)}\\ 
        & = \frac{m}{n}\cdot(1-(1-\frac{1}{m})^{n}),
        \end{aligned}
    \end{align}
    where the second equality is due to the identity $\binom{n}{k} = \frac{n}{k}\binom{n-1}{k-1}$. The Last equality follows by observing that $\sum_{k=0}^{n-1}\binom{n}{k+1}(\frac{1}{m})^{k+1}\cdot(1-\frac{1}{m})^{n-(k+1)}$ is equal to the probability that a binomial random variable with parameters $n$ and $\frac{1}{m}$ equals to some $k$ between $1$ and $n$, i.e., it equals to the probability that a binomial random variable with parameters $n$ and $\frac{1}{m}$ is not equal to $0$.

By the independence assumption we get that $v_i(\{\MostValuableItem{i}\})$ is independent of $|\MostValuableAgents{\MostValuableItem{i}}|$ which implies that:
\begin{equation}
    \E_{v \sim \mathcal{F}}\left[\frac{v_i(\{\MostValuableItem{i}\})}{|\MostValuableAgents{\MostValuableItem{i}}|}\right] = \E_{v \sim \mathcal{F}}[v_i(\{\MostValuableItem{i}\})]\cdot \E_{v \sim \mathcal{F}}\left[\frac{1}{|\MostValuableAgents{\MostValuableItem{i}}|}\right]. \label{eq:v-ind} 
\end{equation}
    Thus, by combining Equation~\ref{expected_value_pr_getting_item} and Equation~\ref{eq:v-ind} we get that the expected welfare of the allocation rule $\AllocRule$ is: 
    $$\E_{v\sim\mathcal{F}}[\sum_{i \in \agents } v_i(\{\MostValuableItem{i}\})]\cdot  \frac{m}{n}\cdot(1-(1-\frac{1}{m})^{n}).$$
    Now, we split the analysis depending on whether $n \geq m$, or $ n<m$.

    \paragraph{Case 1: $n\geq m$.} In this case $ \frac{m}{n}\cdot(1-(1-\frac{1}{m})^{n}) \geq \frac{m}{n}\cdot(1-(1-\frac{1}{m})^{m}) \geq \frac{m}{n}\cdot(1-\frac{1}{e})$, and so we get:
    $$
    \E_{v\sim\mathcal{F}}[\sw{\agents}{\items}] %\geq \E_{v\sim\mathcal{F}}[\sum_{i \in \agents } v_i(\{\MostValuableItem{i}\})]\cdot  \frac{m}{n}\cdot(1-(1-\frac{1}{m})^{n})
    \geq  \E_{v\sim\mathcal{F}}[\sum_{i \in \agents } v_i(\{\MostValuableItem{i}\})]\cdot  \frac{m}{n} \cdot (1-\frac{1}{e}).
    $$
    \paragraph{Case 2: $n < m$.} In this case $ \frac{m}{n}\cdot(1-(1-\frac{1}{m})^{n}) \geq \frac{m}{n}\cdot(1-\frac{1}{e}^{\frac{n}{m}})$. Let $f(x)= x\cdot(1-e^{-\frac{1}{x}})$, and observe that this is an increasing function for $x \geq 0$. Since $n<m$, we have that $ \frac{m}{n}\cdot(1-\frac{1}{e}^{\frac{n}{m}}) >f(1) = 1-\frac{1}{e}$. Overall:
    $$
    \E_{v\sim\mathcal{F}}[\sw{\agents}{\items}] \geq \E_{v\sim\mathcal{F}}[\sum_{i \in \agents } v_i(\{\MostValuableItem{i}\})]\cdot  \frac{m}{n}\cdot(1-(1-\frac{1}{m})^{n}) \geq  \E_{v\sim\mathcal{F}}[\sum_{i \in \agents } v_i(\{\MostValuableItem{i}\})]\cdot (1-\frac{1}{e}).
    $$
    This concludes the proof of the lemma.    
\end{proof}
    
    % By Lemma~\ref{lem:welfare-guarantee}, it is enough to prove that $\frac{\mathbb{E}_{v \sim \mathcal{F}}[\sw{N}{(\copiesmoreagentsTwo)\cdot\items}]}{\copiesmoreagentsTwo} \leq \frac{1}{2} \cdot \mathbb{E}_{v \sim \mathcal{F}}[\sw{N}{\items}]$. From Lemma~\ref{shared-bound}, we get that $\E_{v\sim\mathcal{F}}[\sw{\agents}{\items}]\cdot \frac{1}{2}\geq \frac{\E_{v\sim\mathcal{F}}[\sum_{i \in \agents } v_i(\{\MostValuableItem{i}\})]}{2\cdot \sharedconst\cdot \frac{n}{m}}$, and since $\E_{v\sim\mathcal{F}}[\sum_{i \in \agents } v_i(\{\MostValuableItem{i}\})] \geq \mathbb{E}_{v \sim \mathcal{F}}[\sw{N}{(\copiesmoreagentsTwo)\cdot\items}]$, the claim follows. 

    % \paragraph{Case 2: $n < m$.}
    % For this case, we rum Mechanism~\ref{algo:vcg-copies} with parameters $r=\copiesmoreitems, \, q=1$, and subroutine $B$ for unit demand agents (as defined in \nameref{unit-demand-subroutine}). Similarly to the first case we get that by Lemma~\ref{lem:welfare-guarantee}, it is enough to prove that $\frac{\mathbb{E}_{v \sim \mathcal{F}[\sw{N}{\copiesmoreitems\cdot\items}]}}{\copiesmoreitems} \leq \frac{1}{2} \cdot \mathbb{E}_{v \sim \mathcal{F}}[\sw{N}{\items}]$, which follows directly from Lemma~\ref{shared-bound}.
    
    
    % We now bound $\sw{N}{\items}$ from below, using  Lemma~\ref{more-agents-than-items}. Let $G$ be the event that at least $\minnumofgoodbins$ of the items are most valuable to at most $\maxagentssamebin$ agents and at least $\minagentssamebin$ agents, this set of items depends on the valuation profile $v$ and we denote this set by $E_v$. By Lemma~\ref{more-agents-than-items}, the probability that $G$ occurs is at least $\prmoreagents$. Consider the following (non-truthful) allocation rule $a$: for a valuation profile $v$, if the event $G$ occurs, we allocate only the items that belong to the set $E_v$, i.e., they are most valuable to at most $\maxagentssamebin$ agents and at least $\minagentssamebin$, and each such item is allocated to one of the agents for which it is most valuable uniformly at random. If $G$ doesn't occur, we do not allocate the items.
    % Now, the expected welfare of agent $i$ under the allocation rule $a$ is at least: $$\prmoreagents\cdot \frac{1}{100}\cdot\frac{1}{\maxagentssamebin}\cdot\mathbb E[\max_{j \in [m]}v_i(\{ j \})].$$
    % $\prmoreagents$ is a lower bound on the probability that $G$ occurs. If $G$ occurs, the number of agents whose most valuable item is in $E_v$ is at least $\minagentssamebin\cdot\minnumofgoodbins$, and so by the independence assumption, the probability that agent $i$'s most valuable item belongs to $E_v$ is at least $\frac{1}{100}$. If agent $i$'s most valuable item $j$ belongs to $E_v$ then he gets it with a probability that is proportionate to the number of agents whose most valuable item is also the same, which is at most $\maxagentssamebin$.  

    % Now, the social welfare is at least as large as the welfare of the allocation $a$, and so for $\copiesmoreagentsconst \geq 1000$:
    % $$\mathbb{E}[\sw{N}{\items}] \geq \prmoreagents\cdot\frac{\mathbb E[\sum_{i\in [n]}\max_{j \in [m]}v_i(\{j\})]}{100 \cdot\maxagentssamebin} \geq  2\cdot\frac{\mathbb{E}[\sw{N}{(\frac{\copiesmoreagentsconst n}{m})\cdot\items}]}{\frac{\copiesmoreagentsconst n}{m}}.$$ 



    % We now bound $\sw{N}{\items}$ from below, using  Lemma~\ref{more-items-than-agents}. Let $H$ be the event that at least $\minnumofgoodagens$ of the agents have the same most valuable item as at most $\maxagentssameitem$ other agents, by Lemma~\ref{more-agents-than-items}, $H$ occurs with a probability of at least $\prmoreagentsmoreitems$. Consider the following (non-truthful) allocation rule $a$: for a valuation profile $v$, if the event $H$ occurs, we allocate only the items that are most valuable by at most $\maxagentssameitem$ agents, and each such item is allocated to one of the agents for which it is most valuable uniformly at random. If $H$ doesn't occur, we do not allocate the items.
    % Now, the expected welfare of agent $i$ under the allocation rule $a$ is at least: $$\prmoreagentsmoreitems\cdot \frac{n}{\minnumofgoodagens}\cdot\frac{1}{\maxagentssameitem}\cdot\mathbb E[\max_{j \in [m]}v_i(\{ j \})].$$
    % $\prmoreagents$ is a lower bound on the probability that $H$ occurs. If $H$ occurs, the number of agents whose most valuable is the same as at most $\maxagentssameitem$ agents is at least $\minnumofgoodagens$, and so by the independence assumption, the probability that agent $i$ is such is at least $\frac{n}{\minnumofgoodagens}$. If agent $i$'s most valuable item $j$ is the same as at most $\maxagentssameitem$ other agents, then he gets it with a probability that is proportionate to the number of agents whose most valuable item is also $j$, which is at most $\maxagentssameitem$. 
    
    % Now, the social welfare is at least as large as the welfare of the allocation $a$, and so for $\copiesmoreitems \geq ?$:
    % $$\mathbb{E}[\sw{N}{\items}] \geq \prmoreagentsmoreitems\cdot\frac{\mathbb E[\sum_{i\in [n]}\max_{j \in [m]}v_i(\{j\})]}{10 \cdot\maxagentssameitem} \geq  2\cdot\frac{\mathbb{E}[\sw{N}{(\frac{\copiesmoreitems n}{m})\cdot\items}]}{\copiesmoreitems}.$$ 


    
    
   

    
    % To analyze $\sw{N}{\items}$, we consider the balls and bins problem \anote{add citation} where each ball is an agent and each bin is an item. An agent $i$ belongs to bin $j$ if his most valuable item is $j$.
    % The distribution of balls (agents) into bins (item) is i.i.d with uniform distribution over the bins. 
    % We will be interested in the distribution of the loads between the bins, as it will be used to bound $\sw{N}{2^r\cdot [m]}$ with respect to $\sw{N}{[m]}$.
         
    % In the first case, $n \geq 4m \log_2 m$, and so the number of agents is much larger than the number of items. 
    % \begin{lemma} \label{heavy-loaded-maximum-load-is-expectation}
    % For every $n \geq 4m\log_2m$, the maximum number of agents whose most valuable item 
    % is the same is at most $\frac{en}{m}$ with probability at least $1-\frac{1}{2n}$.   \end{lemma}
    
    % In the second case, $n < 4m \log_2 m$. First, we assume that $n \geq m$.


    
    % We consider each agent's most valuable item, and count how many agents have the same most valuable item. This is equivalent to the balls into bins problem \anote{add citation} as the probability that a certain item is most valuable by some agent $i$ is $\frac{1}{m}$ and is independent of the other agents. we are interested in the maximum load - the maximum number of agents whose most valuable item is the same.     
    % We split the analysis into two cases, in the first $n \leq m\cdot \log m$ (harder case, with ), and in the second case $n \geq m\cdot \log m$ (this case is just by analyzing maximum load). 

% \begin{proof}[Proof of Lemma~\ref{shared-bound}]
%     Consider the allocation rule $\AllocRule$: For a valuation profile $v$, $\AllocRule$ allocates each item $j$ to one of the agents in $\MostValuableAgents{j}$ uniformly at random.    
%     To prove this lemma we bound the expected social welfare by the expected welfare of the allocation rule $\AllocRule$.
%     The expected welfare of an agent $i$ under allocation rule $\AllocRule$ is equal to $\E_{v \sim \mathcal{F}}\left[\frac{v_i(\{\MostValuableItem{i}\})}{|\MostValuableAgents{\MostValuableItem{i}}|}\right]$. We next analyze the random variable of $|\MostValuableAgents{\MostValuableItem{i}}|$. We know that by definition $i \in\MostValuableAgents{\MostValuableItem{i}}$, and 
%     by the \assumption assumption we have that for every $
%     i'\in \agents \setminus \{i\}$, it holds that $\Pr[i'\in \MostValuableAgents{\MostValuableItem{i}} ] = \frac{1}{m}$. Combining with the independent assumption, we get that  $\mid \MostValuableAgents{\MostValuableItem{i}}\mid $ is distributed as  
%       $1+ Bin(n-1, \frac{1}{m})$. Next we analyze the expected value of  $\frac{1}{\mid \MostValuableAgents{\MostValuableItem{i}}\mid}$.

%     \begin{align} \label{expected_value_pr_getting_item}
%         \begin{aligned}
%         \E\left[\frac{1}{\mid \MostValuableAgents{\MostValuableItem{i}}\mid}\right]& =\sum_{k=0}^{n-1}\frac{1}{k+1}\binom{n-1}{k}(\frac{1}{m})^k\cdot(1-\frac{1}{m})^{n-1-k}  \\
%         &= \sum_{k=0}^{n-1}\frac{1}{n}\binom{n}{k+1}(\frac{1}{m})^{k}\cdot(1-\frac{1}{m})^{n-(k+1)} \\ &= \frac{m}{n}\sum_{k=0}^{n-1}\binom{n}{k+1}(\frac{1}{m})^{k+1}\cdot(1-\frac{1}{m})^{n-(k+1)}\\ 
%         & = \frac{m}{n}\cdot(1-(1-\frac{1}{m})^{n}),
%         \end{aligned}
%     \end{align}
%     where the second equality is due to the identity $\binom{n}{k} = \frac{n}{k}\binom{n-1}{k-1}$. The Last equality follows by observing that $\sum_{k=0}^{n-1}\binom{n}{k+1}(\frac{1}{m})^{k+1}\cdot(1-\frac{1}{m})^{n-(k+1)}$ is equal to the probability that a binomial random variable with parameters $n$ and $\frac{1}{m}$ equals to some $k$ between $1$ and $n$, i.e., it equals to the probability that a binomial random variable with parameters $n$ and $\frac{1}{m}$ is not equal to $0$.

% By the independence assumption we get that $v_i(\{\MostValuableItem{i}\})$ is independent of $|\MostValuableAgents{\MostValuableItem{i}}|$ which implies that:
% \begin{equation}
%     \E_{v \sim \mathcal{F}}\left[\frac{v_i(\{\MostValuableItem{i}\})}{|\MostValuableAgents{\MostValuableItem{i}}|}\right] = \E_{v \sim \mathcal{F}}[v_i(\{\MostValuableItem{i}\})]\cdot \E_{v \sim \mathcal{F}}\left[\frac{1}{|\MostValuableAgents{\MostValuableItem{i}}|}\right]. \label{eq:v-ind} 
% \end{equation}
%     Thus, by combining Equation~\ref{expected_value_pr_getting_item} and Equation~\ref{eq:v-ind} we get that the expected welfare of the allocation rule $\AllocRule$ is: 
%     $$\E_{v\sim\mathcal{F}}[\sum_{i \in \agents } v_i(\{\MostValuableItem{i}\})]\cdot  \frac{m}{n}\cdot(1-(1-\frac{1}{m})^{n}).$$
%     Now, we split the analysis depending on whether $n \geq m$, or $ n<m$.

%     \paragraph{Case 1: $n\geq m$.} In this case $ \frac{m}{n}\cdot(1-(1-\frac{1}{m})^{n}) \geq \frac{m}{n}\cdot(1-(1-\frac{1}{m})^{m}) \geq \frac{m}{n}\cdot(1-\frac{1}{e})$, and so we get:
%     $$
%     \E_{v\sim\mathcal{F}}[\sw{\agents}{\items}] %\geq \E_{v\sim\mathcal{F}}[\sum_{i \in \agents } v_i(\{\MostValuableItem{i}\})]\cdot  \frac{m}{n}\cdot(1-(1-\frac{1}{m})^{n})
%     \geq  \E_{v\sim\mathcal{F}}[\sum_{i \in \agents } v_i(\{\MostValuableItem{i}\})]\cdot  \frac{m}{n} \cdot (1-\frac{1}{e}).
%     $$
%     \paragraph{Case 2: $n < m$.} In this case $ \frac{m}{n}\cdot(1-(1-\frac{1}{m})^{n}) \geq \frac{m}{n}\cdot(1-\frac{1}{e}^{\frac{n}{m}})$. Let $f(x)= x\cdot(1-e^{-\frac{1}{x}})$, and observe that this is an increasing function for $x \geq 0$. Since $n<m$, we have that $ \frac{m}{n}\cdot(1-\frac{1}{e}^{\frac{n}{m}}) >f(1) = 1-\frac{1}{e}$. Overall:
%     $$
%     \E_{v\sim\mathcal{F}}[\sw{\agents}{\items}] \geq \E_{v\sim\mathcal{F}}[\sum_{i \in \agents } v_i(\{\MostValuableItem{i}\})]\cdot  \frac{m}{n}\cdot(1-(1-\frac{1}{m})^{n}) \geq  \E_{v\sim\mathcal{F}}[\sum_{i \in \agents } v_i(\{\MostValuableItem{i}\})]\cdot (1-\frac{1}{e}).
%     $$
%     This concludes the proof of the lemma.    
% \end{proof}


